Malicious cryptocurrency miners: Status and Outlook

In this study, we examine the behavior and profitability of modern malware that mines cryptocurrency. Unlike previous studies, we look at the cryptocurrency market as a whole, rather than just Bitcoin. We not only consider PCs, but also mobile phones, and IoT devices. In the past few years, criminals have attacked all these platforms for the purpose of cryptocurrency mining. The question is: how much money do they make? It is common knowledge that mining Bitcoin is now very difficult, so why do the criminals even target low-end devices for mining purposes? By analyzing the most important families of malicious cryptocurrency miners that were active between 2014 and 2017, we are able to report how they work, which currency they mine, and how profitable it is to do so. We will see that the evolution of the cryptocurrency market with many new cryptocurrencies that are still CPU minable and offer better privacy to criminals and have contributed to making mining malware attractive again -- with attackers generating a continuous stream of profit that in some cases may reach in the millions.

==> sections/attack.tex <==

%-----------------------------------------------------------------------------------------------------------------------------------
%							Summary of Bypassing 2FA
%							------------------------ 
%We analyse how this can be exploited to bypass 2FA
%
%---------------------------------------------------------------------------------------------------------------------------------------------
\section{Adversary Model}
\label{sec:attack}



